Object Propagation via Inter-Frame Attentions for Temporally Stable Video Instance Segmentation

Video instance segmentation aims to detect, segment, and track objects in a video. Current approaches extend image-level segmentation algorithms to the temporal domain. However, this results in temporally inconsistent masks. In this work, we identify the mask quality due to temporal stability as a performance bottleneck. Motivated by this, we propose a video instance segmentation method that alleviates the problem due to missing detections. Since this cannot be solved simply using spatial information, we leverage temporal context using inter-frame attentions. This allows our network to refocus on missing objects using box predictions from the neighbouring frame, thereby overcoming missing detections. Our method significantly outperforms previous state-of-the-art algorithms using the Mask R-CNN backbone, by achieving 36.0% mAP on the YouTube-VIS benchmark. Additionally, our method is completely online and requires no future frames. Our code is publicly available at https://github.com/anirudh-chakravarthy/ObjProp.

==> 2_related.tex <==
\section{Related Works}
% There are a couple of research topics similar to video instance segmentation; image instance segmentation, video object segmentation, and object tracking.
% However, image instance segmentation does not use temporal information. While video object segmentation algorithms segment and track a target object, they lack detection of objects. Also, object tracking does not conduct segmentation in general.


% \input{fig-tex/fig_model_init.tex}
% We review conventional video instance segmentation algorithms. We also introduce previous video object segmentation methods, since their aim is similar to video instance segmentation. 

\bfsection{Video Instance Segmentation}
% There are two benchmark datasets for video instance segmentation; YouTube-VIS~\cite{yang2019Video} and MOTS~\cite{voigtlaender2019MOTS}.
With the release of YouTube-VIS~\cite{yang2019Video}, several video instance segmentation has been developed based on MaskR-CNN, which is an object instance segmentation method for images. TrackR-CNN~\cite{voigtlaender2019MOTS} adopts 3D convolutions to the encoder of Mask R-CNN to exploit temporal features from adjacent frames. To track detected objects, TrackR-CNN measures similarities of objects between frames using embeddings from RoI align.
MaskTrackR-CNN~\cite{yang2019Video} has a tracking head, which yields semantic representations of detected objects. MaskTrackR-CNN conducts matching between outputs from the tracking head across frames to agglomerate a track of segmentation masks. 
STEm-Seg~\cite{athar2020STEmSeg} predicts a heat map for each object and models Gaussian distributions across frames to output mask tubes. 
VAE-VIS~\cite{lin2020Video} extracts richer features by training the main decoder for video instance segmentation as well as two auxiliary decoders, each of which performs future frame reconstruction and object detection, respectively.
MaskProp~\cite{bertasius2020Classifying} propagates masks between neighboring frames using deformable convolutions~\cite{dai2017Deformable}. 
SipMask~\cite{cao2020SipMask} delineates adjacent objects using spatial coefficients for each bounding box which improves mask quality.

% However, the previous video instance segmentation methods focus on improving segmentation results. There is a lack of interest in improving bounding boxes. In this work, we shed lights on the importance of the bounding box quality.


% \bfsection{Image Instance Segmentation}
% With the development of a two-stage detector~\cite{ren2015Faster}, researchers have developed many 2D object instance segmentation methods. Mask R-CNN~\cite{he2017Mask} is the most well-known method, which adds a mask head to Faster R-CNN~\cite{ren2015Faster}. There have been many attempts to improve Mask R-CNN's performance by aggregating features~\cite{liu2018Path} or adding more stages for bounding box refinement~\cite{cai2019Cascade,chen2019Hybrid}. 
% Since two-stage detectors are usually not executable in real-time, there are a couple of methods based on one-stage pipeline~\cite{bolya2019Yolact,fu2019RetinaMask} to accelerate a running speed.

% Since video instance segmentation algorithms~\cite{yang2019Video,athar2020STEmSeg,lin2020Video} based on Mask R-CNN have shown promising segmentation quality, we also use it as our baseline.

% \bfsection{Video Object Segmentation}
% There are two types of video object segmentation methods; semi-supervised and unsupervised. Semi-supervised video object segmentation algorithms segment and track a target object annotated by a user at the first frame. 
% % Early algorithms~\cite{ren2007Tracking,jain2014Supervoxelconsistent,wen2015Jots} adopt superpixels and optical flows to propagate a segmentation mask to subsequent frames. 
% With the development of deep learning and the release of DAVIS dataset~\cite{perazzi2016benchmark}, many deep learning-based algorithms have been announced~\cite{jang2017Online,caelles2017Oneshot,perazzi2017Learning}. Early algorithms~\cite{caelles2017Oneshot,luiten2018Premvos,perazzi2017Learning,xu2018Youtubevos} finetune models during inference, called online learning, to segment masks based on the first frame annotations. However, online learning is time-consuming. To tackle this problem, many light-weight video object segmentation algorithms have been developed~\cite{hu2018Videomatch,wugoh2018Fast,oh2019Video,voigtlaender2019Feelvos,zhang2020Transductive,robinson2020Learning,wang2019Ranet}. Most of them suggests performing feature matching between frames to track and segment a target object. 

% However, semi-supervised video object segmentation algorithms require human annotation in the first frame, which is not viable in video instance segmentation.

% Unsupervised video object segmentation aims at discovering salient or primary objects in a video. There are a couple of methods~\cite{wang2019Learning,li2018Instance} that conduct saliency detection to segment salient objects. Another branch of unsupervised object segmentation is matching-based co-segmentation~\cite{yang2019Anchor,wang2019Zeroshot,lu2019See}. They segment objects that consistently appear across frames. 

% However, unsupervised video object segmentation methods can only segment salient objects and do not classify object classes.

% \bfsection{Multi-object Tracking}

\bfsection{Attention Model}
The attention mechanism was first introduced by Bahdanau~\etal~\cite{Bahdanau2015attention} for text summarization using a neural transduction model. Following the success of attention in NLP tasks, several methods have emerged to use attention mechanisms in convolutional neural networks. 
Attention has been used for several image~\cite{ramachandran2019standalone, hu2018relation, bello2019attention} and video recognition~\cite{xiao2018video} tasks. 
The transformer model, first introduced by Vaswani~\etal~\cite{vaswani2017Attention}, also leverages attention mechanisms.

We use an inter-frame attention mechanism to improve temporal stability for video instance segmentation.

% \wj{Add description that we use the attention model to improve temporal stability}

% \bfsection{Transformers}
% The transformer is a machine learning model that leverages attention mechanisms.
% Vaswani~\etal~\cite{vaswani2017Attention} first introduced the transformer with multi-head attention modules.  BERT~\cite{devlin2018Bert} adopts a bidirectional encoder in the transformer.
% Recently, researchers started applying the transformer to object detection problems. 
% DETR~\cite{carion2020Endtoend} is an object detection algorithm based on the transformer. 
% Zhu~\etal~\cite{zhu2020Deformable} developed a deformable DETR, which exploits deformable convolutions to accelerate DETR.


